BaThe: Defense against the Jailbreak Attack in Multimodal Large Language Models by Treating Harmful Instruction as Backdoor Trigger

Multimodal Large Language Models (MLLMs) have showcased impressive performance in a variety of multimodal tasks. On the other hand, the integration of additional image modality may allow the malicious users to inject harmful content inside the images for jailbreaking. Unlike text-based LLMs, where adversaries need to select discrete tokens to conceal their malicious intent using specific algorithms, the continuous nature of image signals provides a direct opportunity for adversaries to inject harmful intentions. In this work, we propose $\textbf{BaThe}$ ($\textbf{Ba}$ckdoor $\textbf{T}$rigger S$\textbf{h}$i$\textbf{e}$ld), a simple yet effective jailbreak defense mechanism. Our work is motivated by recent research on jailbreak backdoor attack and virtual prompt backdoor attack in generative language models. Jailbreak backdoor attack uses harmful instructions combined with manually crafted strings as triggers to make the backdoored model generate prohibited responses. We assume that harmful instructions can function as triggers, and if we alternatively set rejection responses as the triggered response, the backdoored model then can defend against jailbreak attacks. We achieve this by utilizing virtual rejection prompt, similar to the virtual prompt backdoor attack. We embed the virtual rejection prompt into the soft text embeddings, which we call ``wedge''. Our comprehensive experiments demonstrate that BaThe effectively mitigates various types of jailbreak attacks and is adaptable to defend against unseen attacks, with minimal impact on MLLMs' performance.

==> 6-checklist.tex <==

\newcommand{\yes}{\textcolor{black}{Yes.}\xspace}
\newcommand{\no}{\textcolor{black}{No.}\xspace}
\newcommand{\na}{\textcolor{black}{NA.}\xspace}
\newcommand{\pa}{\textcolor{black}{Partial.}\xspace}


\section{Checklist}
This paper:
\begin{itemize}
    \item Includes a conceptual outline and/or pseudocode description of AI methods introduced (yes/partial/no/NA)
    
    \yes
    
\item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results (yes/no)

\yes

\item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper (yes/no)

\yes

\end{itemize}

\begin{itemize}
    \item Does this paper make theoretical contributions? (yes/no)
    
    \no
\end{itemize}




\begin{itemize}
    \item Does this paper rely on one or more datasets? 
    
    \yes

If yes, please complete the list below.

1.JailbreakV-28 \cite{luo2024jailbreakv}

2.LLaVA-Instruct-150K \cite{liu2024visual}

3.FigStep \cite{gong2023figstep}

4.Query-related \cite{liu2023query}

5.HADES \cite{li2024images}
\end{itemize}



\begin{itemize}

\item A motivation is given for why the experiments are conducted on the selected datasets (yes/partial/no/NA)

\yes

\item All novel datasets introduced in this paper are included in a data appendix. (yes/partial/no/NA)

\no

\item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no/NA)

\yes

\item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. (yes/no/NA)

\yes

\item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. (yes/partial/no/NA)

\yes


\item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. (yes/partial/no/NA)

\na

\end{itemize}


\begin{itemize}
    \item Does this paper include computational experiments? (yes/no)

\yes

If yes, please complete the list below.

See Experiments Section.
\end{itemize}

\begin{itemize}
\item Any code required for pre-processing data is included in the appendix. (yes/partial/no).

\no



\item All source code required for conducting and analyzing the experiments is included in a code appendix. (yes/partial/no)

\no


\item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no)

\yes

\item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from (yes/partial/no)

\yes


\item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. (yes/partial/no/NA)

\yes

\item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. (yes/partial/no)

\yes

\item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. (yes/partial/no)

\yes

\item This paper states the number of algorithm runs used to compute each reported result. (yes/no)

\yes

\item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. (yes/no)

\yes

\item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). (yes/partial/no)

\no

\item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. (yes/partial/no/NA)

\yes

\item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. (yes/partial/no/NA)

\no


\end{itemize}

